Path homology and temporal networks

We present an algorithm to compute path homology for simple digraphs, and use it to topologically analyze various small digraphs en route to an analysis of complex temporal networks which exhibit such digraphs as underlying motifs. The digraphs analyzed include all digraphs, directed acyclic graphs, and undirected graphs up to certain numbers of vertices, as well as some specially constructed cases. Using information from this analysis, we identify small digraphs contributing to path homology in dimension $2$ for three temporal networks, and relate these digraphs to network behavior. We conclude that path homology can provide insight into temporal network structure and vice versa.

==> commands.tex <==

% blackboard bold for naturals, integers, etc.
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

% editing

%comments not shown
%\newcommand{\samir}[1]{}
%\newcommand{\matvey}[1]{}
%\newcommand{\steve}[1]{}

%comments shown
\newcommand{\samir}[1]{\textcolor{purple}{Samir says: {#1}}}
\newcommand{\matvey}[1]{\textcolor{red}{Matvey says: {#1}}}
\newcommand{\steve}[1]{\textcolor{green}{Steve says: {#1}}}





% text commands
\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbb}
\newcommand{\mf}{\mathfrak}
\newcommand{\tn}[1]{\textnormal{#1}}


% greek lower case
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\w}{\omega}
\newcommand{\s}{\sigma}
\newcommand{\ph}{\varphi}
\newcommand{\p}{\partial}
\renewcommand{\t}{\tau}
\renewcommand{\th}{\theta}
\newcommand{\z}{\zeta}

% greek upper case
\newcommand{\Om}{\Omega}
\newcommand{\Ga}{\Gamma}
\newcommand{\Si}{\Sigma}
\newcommand{\La}{\Lambda}

% script upper case
\newcommand{\A}{\mathscr{A}}
\newcommand{\B}{\mathscr{B}}


%% counter for labels in description env
\newcounter{desccount}
\newcommand{\descitem}[1]{%
  \item[#1] \refstepcounter{desccount}\label{#1}
}
\newcommand{\descref}[1]{\hyperref[#1]{#1}}


% pullback functions
\newcommand{\fst}{f^{*}}
\newcommand{\gst}{g^{*}}


% misc

\newcommand{\uniflim}{\operatorname{unif}\lim}
\newcommand{\unifr}{\xrightarrow{\operatorname{unif.}}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\hr}{\hookrightarrow}
\newcommand{\li}{\lambda_I}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lbar}{\left|}
\newcommand{\rbar}{\right|}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}

\newcommand\mattwo[4]{\left(\begin{smallmatrix}
			{#1} & {#2}\\
     			{#3} & {#4}
                     \end{smallmatrix}\right)}
\newcommand\mattres[9]{\left(\begin{smallmatrix}
			{#1} & {#2}&{#3}\\
     			{#4} & {#5}&{#6}\\
     				{#7} &{#8} &{#9}
                     \end{smallmatrix}\right)}
                     
\newcommand{\linf}{l^{\infty}}		%l-infinity norm
\newcommand{\borel}{\operatorname{Borel}}	
\newcommand{\fa}{\forall}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\ip}[2]{\left\la #1,#2 \right\ra}
\renewcommand{\o}{\overline}
\renewcommand{\u}{\underline}
\newcommand{\h}{\hat}
\renewcommand{\r}{\rightarrow}
\newcommand{\xr}{\xrightarrow}
\newcommand{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\de}[2]{\frac{d #1}{d #2}}
\newcommand{\ddx}{\frac{d}{dx}}
\newcommand{\norm}[1]{\|#1\|} 
\newcommand{\tnorm}[1]{||#1||} % two-norm, i.e., with two bars
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\rw}{\rightharpoonup}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\pair}[1]{\left(#1\right)}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\wh}{\widehat}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\pv}{\operatorname{PV}}
\newcommand{\curl}{\operatorname{curl}}
\newcommand{\ds}{\displaystyle}
\newcommand{\inv}{^{-1}}
\newcommand{\dg}[1]{\textnormal{deg(#1)}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\ind}{\operatorname{Ind}}
\newcommand{\im}{\operatorname{im}}

%% In an integral, for the differential term
%\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\diff}{\, d}
%% For denoting powers of a differential term
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

%% integral with space removed
\newcommand{\myint}{\int\!}

\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceil }
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor }


%% PH stuff?
\newcommand{\pathhom}{\mathbf{PathHom}}
\newcommand{\dfchom}{\mathbf{DFCHom}}

\newcommand{\mlp}[1]{K^{\rightarrow}_{n_1,\ldots,n_{#1}}} 
\newcommand{\mlpgraph}[1]{K_{n_1,\ldots,n_{#1}}} 


\newcommand{\db}{d_{\operatorname{B}}}
\newcommand{\dgm}{\operatorname{Dgm}}
\newcommand{\vr}{\operatorname{VR}}
\newcommand{\cech}{\check{\operatorname{C}}}
\newcommand{\pvec}{{\operatorname{\mathbf{PVec}}}}
\newcommand{\pers}{{\operatorname{\mathbf{Pers}}}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\di}{d_{\operatorname{I}}}

\newcommand{\src}{\mf{D}^{\operatorname{so}}}
\newcommand{\sink}{\mf{D}^{\operatorname{si}}}

\newcommand{\so}{\operatorname{so}}
\newcommand{\si}{\operatorname{si}}



\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}


\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{defn}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem*{comments}{Comments}
%

\newenvironment{subproof}[1][\proofname]{%
  \renewcommand{\qedsymbol}{$\blacksquare$}%
  \begin{proof}[#1]%
}{%
  \end{proof}%
}

%% for align right within equation
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother



==> packages.tex <==


\usepackage{arxiv}

\usepackage{booktabs} 
\usepackage{nicefrac}  
\usepackage{microtype}
\usepackage[utf8]{inputenc}

%\usepackage{enumitem}
%\usepackage{times}
%\usepackage{amsaddr}
%\usepackage[margin=1in]{geometry}

\usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{multirow}

%\usepackage{url}
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage[normalem]{ulem}
%\usepackage{mathabx}
\usepackage{bbm}
\usepackage{array}
\usepackage[colorlinks=true,urlcolor=purple,
linkcolor=purple,citecolor=purple]{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{float}


\usepackage{mathrsfs}
%\usepackage{framed}
%\usepackage{latexsym}
%\usepackage{pb-diagram}
%\usepackage[mathscr]{}
\usepackage{graphicx}
%\usepackage[all]{xy} 
\usepackage{color}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{thmtools,thm-restate} %%for restating results 
%\usepackage[usenames, dvipsnames]{color}

\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\bfseries}}
\makeatother

%% TIK-Z RELATED PACKAGES
\usepackage{tikz}
\usetikzlibrary{decorations.markings, backgrounds, calc, positioning, shapes, shadows, arrows, fit, automata}
\usepackage{tikz-cd}
% Nice arrowheads
\usetikzlibrary{arrows.meta}
%\tikzset{>={Latex[length=3mm,width=2mm]}}
\tikzset{>={Latex}}


